Occluded Human Mesh Recovery

Top-down methods for monocular human mesh recovery have two stages: (1) detect human bounding boxes; (2) treat each bounding box as an independent single-human mesh recovery task. Unfortunately, the single-human assumption does not hold in images with multi-human occlusion and crowding. Consequently, top-down methods have difficulties in recovering accurate 3D human meshes under severe person-person occlusion. To address this, we present Occluded Human Mesh Recovery (OCHMR) - a novel top-down mesh recovery approach that incorporates image spatial context to overcome the limitations of the single-human assumption. The approach is conceptually simple and can be applied to any existing top-down architecture. Along with the input image, we condition the top-down model on spatial context from the image in the form of body-center heatmaps. To reason from the predicted body centermaps, we introduce Contextual Normalization (CoNorm) blocks to adaptively modulate intermediate features of the top-down model. The contextual conditioning helps our model disambiguate between two severely overlapping human bounding-boxes, making it robust to multi-person occlusion. Compared with state-of-the-art methods, OCHMR achieves superior performance on challenging multi-person benchmarks like 3DPW, CrowdPose and OCHuman. Specifically, our proposed contextual reasoning architecture applied to the SPIN model with ResNet-50 backbone results in 75.2 PMPJPE on 3DPW-PC, 23.6 AP on CrowdPose and 37.7 AP on OCHuman datasets, a significant improvement of 6.9 mm, 6.4 AP and 20.8 AP respectively over the baseline. Code and models will be released.

==> tables/conorm_placement.tex <==
\begin{table}[h]
\centering
\small
    \renewcommand{\arraystretch}{1.2}
    \rowcolors{1}{}{lightgray}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{@{}l|c c c c c@{}}
        \Xhline{3\arrayrulewidth}
         & SPIN & Depth 1  & Depth 2  & Depth 3 & Depth 4\\
        MPJPE $\downarrow$ & 128.4  & 114.8 & \textbf{114.0} & 115.6 & 118.4 \\
        PMPJPE $\downarrow$ &  82.1 & 76.7 & \textbf{76.1} & 78.9 & 80.0 \\
        \Xhline{3\arrayrulewidth}
    \end{tabular}
\caption{Comparison of insertion of a single CoNorm block at various depths in the backbone. Context based feature normalization achieved best performance after the second ResNet block.}
\label{table:conorm_placement}
\end{table}


==> tables/introduction.tex <==
\begin{table}[b]
% \captionsetup{font=small}
\small

\begin{center}

\resizebox{3.3in}{!}{
    \setlength{\tabcolsep}{3pt}
    \rowcolors{3}{}{lightgray}
    \begin{tabular}{@{}l|c|c|c @{}}
    \Xhline{3\arrayrulewidth}
    
    \multirow{2}{*}{\textbf{Method}} & \textbf{3DPW-PC } & \textbf{CrowdPose} & \textbf{OCHuman} \\
     & \scriptsize{PMPJPE $\downarrow$} & \scriptsize{AP $\uparrow$} & \scriptsize{AP $\uparrow$} \\
    \hline
    CRMH~\cite{jiang2020coherent} & 103.5 & - & -  \\
    SPIN~\cite{kolotouros2019learning} & 83.7  & 14.8 & 11.1\\
    ROMP-R50$\dagger$~\cite{sun2021monocular} & 79.7 & 18.9 & 15.6 \\
    OCHMR (Ours) & \textbf{77.1 (-2.6)}  & \textbf{21.4 (+2.5)} & \textbf{24.8 (+9.2)}  \\
    
    \hline
    \multicolumn{4}{c}{\scriptsize{Using ground-truth bounding boxes}}\\
    \hline
    SPIN~\cite{kolotouros2019learning} & 82.1  & 17.2 & 16.9\\
    OCHMR (Ours) & \textbf{75.2 (-6.9)}  & \textbf{23.6 (+6.4)} & \textbf{37.7 (+20.8)}  \\
    
    \hline

    \Xhline{1\arrayrulewidth}
    \end{tabular}
}
\caption{OCHMR is implemented by conditioning SPIN with ResNet-50 backbone. We use HRNet-W32~\cite{sun2019deep} for top-down body-center estimation. The relative improvements in  PMPJPE(mm) and AP are reported using Faster R-CNN and ground truth bounding boxes on the \texttt{val} sets. Datasets with more occlusions and crowding demonstrate higher gains. $\dagger$ denotes a bottom-up approach and R-50 denotes a ResNet-50 backbone.}
\label{table:introduction}
\end{center}
\end{table}

==> tables_rebuttal/object_occlusion.tex <==
% \begin{table}[b]
% \captionsetup{font=small}
% \begin{center}

% \resizebox{3.35in}{!}{
%     \small
%     % \setlength{\tabcolsep}{3pt}
%     \renewcommand{\arraystretch}{1.0}
%     \begin{tabular}{@{}l|l|l|l @{}}
%     \Xhline{3\arrayrulewidth}
%          \small{\textbf{Method}} &\small{\texttt{3DPW-OC} $\downarrow$} &\small{\texttt{OCHuman} $\uparrow$}   & \small{\texttt{CrowdPose} $\uparrow$}  \\
%     \hline
%   ROMP (bottom-up)  & 119.7  & 15.6  & 18.9 \\
%   \hline
%   SPIN  & 128.4  & 16.9  & 17.2 \\
%   OCHMR-SPIN  & \textbf{112.2 (-16.2)}  & \textbf{37.7 (+20.8)}  & \textbf{23.6 (+6.4)} \\
%   \hline
%   I2LMeshNet  & 125.7  & 18.1  & 19.0 \\
%   OCHMR-I2LMeshNet  & \textbf{110.0 (-15.7)}  & \textbf{38.0 (+19.9)}  & \textbf{23.7 (+4.7)} \\
%   \hline
%   PyMaf  & 123.6  & 19.3  & 20.8 \\
%   OCHMR-PyMaf  & \textbf{105.8 (-17.8)}  & \textbf{39.1 (+19.8)}  & \textbf{26.3 (+5.5)} \\
%     \Xhline{3\arrayrulewidth}
%     \end{tabular}
% }
% \vspace*{-0.1in}
% \caption{OCHMR with other top-down methods. We report MPJPE (3D) and AP (2D) on the datasets using ground-truth boxes.}
% %  \vspace*{-0.6in}
% \label{table:rebuttal:object_occlusion}
% \end{center}
% \end{table}


\begin{table}[b]
\vspace*{-0.2in}
\captionsetup{font=scriptsize}
\centering
\small
\resizebox{3.35in}{!}{
    \renewcommand{\arraystretch}{1.0}
    % \setlength{\tabcolsep}{1pt}
    \begin{tabular}{@{}l|c c|c c@{}}
        \Xhline{3\arrayrulewidth}
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Person Occlusion}} & \multicolumn{2}{c}{\textbf{Object Occlusion}}  \\
         & \texttt{3DPW-PC $\downarrow$} & \texttt{OCHuman $\uparrow$} & \texttt{3DPW-OCC $\downarrow$} & \texttt{3DOH $\downarrow$}\\
        \hline
        SPIN & 128.4 & 16.9 & 95.6 & 104.3 \\
        ROMP & 119.7 & 15.6 & - & - \\
        HMR-EFT (pose) & 116.4 & 20.8  & 94.4 & 75.2 \\
        PARE & 122.5 & 18.0  & \textbf{90.5} & \textbf{63.3} \\
        OCHMR (Ours) & \textbf{112.2} & \textbf{37.7} & 93.5  & 98.6 \\
        \Xhline{3\arrayrulewidth}
    \end{tabular}
}
\vspace*{-0.1in}
\caption{We report MPJPE/AP of methods under person and object occlusion. Evaluations are done using ground-truth boxes. HMR-EFT uses AlphaPose for 2D pose.}
\label{table:rebuttal:object_occlusion}
\vspace*{-0.5in}
\end{table}


==> tables_rebuttal/other_topdown.tex <==
\begin{table}[t]
\captionsetup{font=scriptsize}
\begin{center}
\vspace*{-0.1in}
\resizebox{3.30in}{!}{
    \small
    % \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{@{}l|l|l|l @{}}
    \Xhline{3\arrayrulewidth}
         \small{\textbf{Method}} &\small{\texttt{3DPW-PC} $\downarrow$} &\small{\texttt{OCHuman} $\uparrow$}   & \small{\texttt{CrowdPose} $\uparrow$}  \\
    \hline
   ROMP \small{(bottom-up)}  & 119.7  & 15.6  & 18.9 \\
   \hline
   SPIN  & 128.4  & 16.9  & 17.2 \\
   OCHMR \small{(\textit{early-fusion})}  & 115.8 & 30.6  & 20.9  \\
   OCHMR ($\mathcal{L}_\text{single}$)  & 116.9  & 32.8  & 20.4 \\
   OCHMR + CAR  & 113.8   & 36.9  & 23.0 \\
   OCHMR (Ours)   & \textbf{112.2 (-16.2)}  & \textbf{37.7 (+20.8)}  & \textbf{23.6 (+6.4)} \\
   \hline
   I2LMeshNet  & 125.7  & 18.1  & 19.0 \\
   \small{OCHMR-I2LMeshNet}  & \textbf{110.0 (-15.7)}  & \textbf{38.0 (+19.9)}  & \textbf{23.7 (+4.7)} \\
   \hline
   PyMaf  & 123.6  & 19.3  & 20.8 \\
   \small{OCHMR-PyMaf} & \textbf{105.8 (-17.8)}  & \textbf{39.1 (+19.8)}  & \textbf{26.3 (+5.5)} \\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
}
\vspace*{-0.1in}
\caption{OCHMR with top-down methods and losses. Metrics are MPJPE/AP.}
 \vspace*{-0.4in}
\label{table:rebuttal:other_topdown}
\end{center}
\end{table}


==> tables_rebuttal/panoptic.tex <==
\begin{table}[b]
\captionsetup{font=scriptsize}
\begin{center}
\vspace*{-0.2in}
\resizebox{2.9in}{!}{
    \small
    % \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{1.0}
    \begin{tabular}{@{}l|llll|l @{}}
    \Xhline{3\arrayrulewidth}
         \small{\textbf{Method}} &\small{\textbf{Haggling}} &\small{\textbf{Mafia}}   & \small{\textbf{Ultim.}} & \small{\textbf{Pizza}} & \small{\textbf{Mean}}  \\
    \hline
   CRMH & 129.6 & 133.5 & 153.0 & 156.7 & 143.2 \\
   ROMP \small{(bottom-up)} & \textbf{111.8} & 129.0 & 148.5 & \textbf{149.1} & 134.6 \\
   SPIN & 124.3 & 132.4 & 150.4 & 153.5 & 140.2 \\
   OCHMR \small{(Ours)} & 115.5 & \textbf{123.7} & \textbf{142.6} & 150.6 & \textbf{133.1} \\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
}
\vspace*{-0.1in}
\caption{We report MPJPE on the CMU-Panoptic benchmark. All methods are trained using same data for a fair comparison.}
 \vspace*{-0.6in}
\label{table:rebuttal:panoptic}
\end{center}
\end{table}

